Adaptation and Robust Learning of Probabilistic Movement Primitives

Probabilistic representations of movement primitives open important new possibilities for machine learning in robotics. These representations are able to capture the variability of the demonstrations from a teacher as a probability distribution over trajectories, providing a sensible region of exploration and the ability to adapt to changes in the robot environment. However, to be able to capture variability and correlations between different joints, a probabilistic movement primitive requires the estimation of a larger number of parameters compared to their deterministic counterparts, that focus on modeling only the mean behavior. In this paper, we make use of prior distributions over the parameters of a probabilistic movement primitive to make robust estimates of the parameters with few training instances. In addition, we introduce general purpose operators to adapt movement primitives in joint and task space. The proposed training method and adaptation operators are tested in a coffee preparation and in robot table tennis task. In the coffee preparation task we evaluate the generalization performance to changes in the location of the coffee grinder and brewing chamber in a target area, achieving the desired behavior after only two demonstrations. In the table tennis task we evaluate the hit and return rates, outperforming previous approaches while using fewer task specific heuristics.

==> fig/convergence/log_cond_sw.tex <==
% This file was created by matplotlib2tikz v0.6.14.
\begin{tikzpicture}

\begin{axis}[
title={Log Condition Number of $\Sigma_w$},
xlabel={Number of samples},
ylabel={$\log{\kappa(\Sigma_w)}$},
xmin=-3.95, xmax=104.95,
ymin=5.19323420630898, ymax=30.7970055973459,
width=\figurewidth,
height=\figureheight,
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black},
legend style={draw=white!80.0!black},
legend entries={{MAP},{MLE}},
legend cell align={left}
]
\addlegendimage{no markers, blue}
\addlegendimage{no markers, red}
\addplot [semithick, blue]
table {%
1 9.13207540164585
2 8.30439101991233
3 7.75394478912242
4 7.33451313866483
5 7.10199361304911
6 6.83754405723635
7 6.80993980449257
8 6.85879748391743
9 6.79259968512425
10 6.90671365872074
11 6.50266383807775
12 6.95619519894821
13 6.74500184439421
14 6.6327999199575
15 6.85502003784865
16 6.63701329081249
17 6.58430825025209
18 6.90661057952875
19 6.5977238387892
20 6.35704199681066
21 6.6716376658144
22 6.50696494949895
23 6.7254125248832
24 6.65063391697787
25 6.84263936246003
26 6.49560066399165
27 6.62024975008634
28 6.61626234371101
29 6.65414349652979
30 6.59583032159432
31 6.61813238993394
32 6.56933820660289
33 6.4053630317408
34 6.73669790594705
35 6.71420812047454
36 6.86201856895587
37 6.82671651991612
38 6.51862419340056
39 6.74757698494401
40 6.57311665078533
41 6.75902674712151
42 6.43141894277008
43 6.46732969733098
44 6.66026916304138
45 6.77698309180274
46 6.49461400078821
47 6.7191026316082
48 6.68475676811049
49 6.6785929882278
50 6.76181318106123
51 6.70214163347979
52 6.63338954789053
53 6.71789581880134
54 6.69230174872596
55 6.67332490312661
56 6.72406900121395
57 6.86543525332209
58 6.52263725352639
59 6.63848892276133
60 6.56198604913815
61 6.62348610693718
62 6.61233720122443
63 6.75907403470285
64 6.74971308209363
65 6.87370443042132
66 6.71175357783751
67 6.67569273061272
68 6.66752140171763
69 6.64333429570902
70 6.76808325790202
71 6.64215090190416
72 6.87758055354054
73 6.65709271490995
74 6.67693725818221
75 6.61485149094542
76 6.82414258574359
77 6.87979911525448
78 6.80082840723281
79 6.81975595434711
80 6.86960200511922
81 6.73454176182252
82 6.92680058408337
83 6.7730751484202
84 6.77486539982096
85 6.76091458750647
86 6.7602874623611
87 6.71977027461335
88 6.72353075639897
89 6.67660810200778
90 6.75630317534818
91 6.81630868782453
92 6.62387738766595
93 6.73970788468543
94 6.74757136604215
95 6.70875618063958
96 6.79347564333255
97 6.79846468338832
98 6.8395805558012
99 6.86473165778155
100 6.82851485726053
};
\addplot [semithick, red]
table {%
2 29.6331978068443
3 29.0776143206821
4 28.8662274301515
5 28.4162790400574
6 28.1268053934089
7 28.5367866374433
8 27.933936249128
9 27.7139708167204
10 27.7543805865991
11 27.3624412466025
12 27.1607283119111
13 27.0124747666363
14 27.2405152656819
15 26.8348755433784
16 26.6466734915961
17 26.2010741000501
18 25.8983032446342
19 25.9905337608245
20 26.004849437245
21 25.4250785882187
22 25.670321049466
23 25.3288948725374
24 25.2197508755816
25 24.9808448828166
26 25.1625152381117
27 24.6146152368876
28 24.3643683939588
29 24.0893113221794
30 24.0311800920377
31 23.650393352234
32 23.690389896094
33 22.9185270917414
34 23.2130973544648
35 22.1125916900283
36 13.3710037180071
37 12.6219915097433
38 11.6441934462344
39 11.1191310194151
40 10.7652862746258
41 10.3260217853605
42 10.2269769924934
43 10.0499895145309
44 9.8917665183345
45 9.53030239320366
46 9.33769491682253
47 9.25058712925422
48 9.44861369979061
49 9.00031267142751
50 9.06564931403333
51 9.0554005218485
52 9.00473840682494
53 9.11908866925677
54 8.76713395795047
55 8.80626632557608
56 8.89615010728745
57 8.67801608141308
58 8.31724789984045
59 8.54923336637813
60 8.51368701548305
61 8.50355407509855
62 8.38657880283481
63 8.39406440645791
64 8.07147946783019
65 8.48189323794304
66 8.28057631757703
67 8.19109741707229
68 8.19205939620159
69 8.1830578556096
70 8.28882233044539
71 8.26636253178598
72 8.2622742818019
73 8.12085014287586
74 7.98718882572127
75 8.21319627380038
76 8.11340486358158
77 8.0957087980735
78 8.14368967295215
79 7.93580269201964
80 8.07222407059122
81 7.99157050885219
82 7.97426272880001
83 8.08321126903707
84 8.01299956667085
85 7.87600330519484
86 7.95810083478377
87 7.88967242621222
88 7.92647122607964
89 7.79333052206889
90 7.93021428829581
91 7.97606181130243
92 7.84189962966065
93 7.98509067596321
94 7.93317808221981
95 7.88309803732631
96 7.85683300731277
97 7.9773619177785
98 7.9577017648024
99 7.73652244967335
100 7.77922164882036
};
\end{axis}

\end{tikzpicture}


==> fig/convergence/mu_w.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
%title={Convergence of $\vect{\mu}_\omega$},
xlabel={Size of training set $n$},
ylabel={Error},
xmin=0, xmax=30,
ymin=0, ymax=1.6,
axis on top,
width=\figurewidth,
height=\figureheight
]

\addplot [red]
table {%
1 1.50714939984747
2 1.03694628087972
3 0.785290313311921
4 0.625329585124036
5 0.517200096267866
6 0.455886569585489
7 0.403873269820708
8 0.365933743519432
9 0.337109658699963
10 0.298966954080273
11 0.278162206689981
12 0.254272554154807
13 0.234442057351096
14 0.231617593751822
15 0.221276822354253
16 0.200818764806325
17 0.210621234069269
18 0.185765134107501
19 0.185225600964966
20 0.163166914560885
21 0.157234181961532
22 0.160912173230511
23 0.172933104280139
24 0.157665379938963
25 0.158049132719536
26 0.133425818670255
27 0.129225073666417
28 0.137693175607451
29 0.128249888342732
30 0.136521454034454
};
\end{axis}

\end{tikzpicture}


==> fig/convergence/sw.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
%title={Convergence of $\matr{\Sigma}_\omega$},
xlabel={Size of training set $n$},
ylabel={Error},
xmin=0, xmax=30,
ymin=0, ymax=1.4,
axis on top,
width=\figurewidth,
height=\figureheight
]
\addplot [red]
table {%
1 1.27652580467245
2 0.555843220927855
3 0.320643547048438
4 0.20966183901719
5 0.150481009559455
6 0.120121867796379
7 0.0965013230066253
8 0.0821637502515701
9 0.0885809525027466
10 0.0635143550512526
11 0.0719624689053914
12 0.0638876559534666
13 0.064959805255737
14 0.0482905316269553
15 0.047965746595645
16 0.0506522503149391
17 0.0508144810248318
18 0.0494414990469037
19 0.0645949237645197
20 0.0447386301175089
21 0.0407369091413954
22 0.0414814322311444
23 0.0383131203561295
24 0.041209154908572
25 0.0457810803315383
26 0.0429565318623357
27 0.0346439727173524
28 0.0350776958118732
29 0.0338926142842054
30 0.0358758684194431
};
\end{axis}

\end{tikzpicture}


==> fig/training/em_iter_lh.tex <==
% This file was created by matplotlib2tikz v0.6.14.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
xlabel={Iterations},
ylabel={Log-Likelihood},
xmin=-0.35, xmax=7.35,
ymin=-13476.7740750738, ymax=283012.255576549,
width=\figurewidth,
height=\figureheight,
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black}
]
\addplot [semithick, color0, forget plot]
table {%
0 0
1 114991.617570796
2 215856.676816035
3 265708.238006764
4 269358.379314241
5 269457.696137116
6 269504.000895061
7 269535.481501476
};
\end{axis}

\end{tikzpicture}

==> fig/training/em_lh.tex <==
% This file was created by matplotlib2tikz v0.6.14.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
xlabel={Iterations},
ylabel={Log-Likelihood},
xmin=-1.45, xmax=30.45,
ymin=-5.76632921991404, ymax=121.092913618195,
width=\figurewidth,
height=\figureheight,
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black}
]
\addplot [semithick, color0, forget plot]
table {%
0 0
1 15.5061404051958
2 28.8603666913114
3 38.8425891693332
4 46.7678883185727
5 53.3550300494535
6 59.0016164194676
7 63.9498769982602
8 68.3581562808249
9 72.3356008100091
10 75.9606667489861
11 79.2917098568287
12 82.3733832511352
13 85.2406775735435
14 87.9215694279992
15 90.4388144892291
16 92.8111962056719
17 95.0544174549286
18 97.1817515370785
19 99.2045270094532
20 101.132495275349
21 102.974113780831
22 104.736767302675
23 106.426943185739
24 108.050371680642
25 109.612139536999
26 111.116782814614
27 112.568363423285
28 113.970532656356
29 115.326584398281
};
\end{axis}

\end{tikzpicture}
